Automatic Dynamic Parallelotope Bundles for Reachability Analysis of Nonlinear Systems

Reachable set computation is an important technique for the verification of safety properties of dynamical systems. In this paper, we investigate reachable set computation for discrete nonlinear systems based on parallelotope bundles. The algorithm relies on computing an upper bound on the supremum of a nonlinear function over a rectangular domain, which has been traditionally done using Bernstein polynomials. We strive to remove the manual step of parallelotope template selection to make the method fully automatic. Furthermore, we show that changing templates dynamically during computations cans improve accuracy. To this end, we investigate two techniques for generating the template directions. The first technique approximates the dynamics as a linear transformation and generates templates using this linear transformation. The second technique uses Principal Component Analysis (PCA) of sample trajectories for generating templates. We have implemented our approach in a Python-based tool called Kaa and improve its performance by two main enhancements. The tool is modular and use two types of global optimization solvers, the first using Bernstein polynomials and the second using NASA's Kodiak nonlinear optimization library. Second, we leverage the natural parallelism of the reachability algorithm and parallelize the Kaa implementation. We demonstrate the improved accuracy of our approach on several standard nonlinear benchmark systems.

==> Makefile <==

MAIN=main

all $(MAIN).pdf : $(MAIN).tex 
	pdflatex $<
	-bibtex $(basename $<)
	pdflatex $<
	pdflatex $<

$(MAIN).fmt : prelude1.tex
	pdflatex -ini -jobname="$(MAIN)" "&pdflatex prelude1.tex\dump"

STEM=$(notdir $(PWD))

snapshot : $(MAIN).pdf
	@TODAY="`date +%Y%m%d`"; \
	N="1"; \
	while [ -f $$TODAY-$(STEM)-$$N.pdf ]; do \
	  N="`expr $$N + 1`"; done; \
	echo $(MAIN).pdf '->' $$TODAY-$(STEM)-$$N.pdf; \
	cp $(MAIN).pdf $$TODAY-$(STEM)-$$N.pdf

%.pdf : %.gpl
	gnuplot $(<)

plots : $(subst gpl,pdf,$(wildcard *.gpl))

clean :
	rm -f $(addprefix $(MAIN)., aux bbl blg fmt log out pdf)

.PHONY : plots snapshot clean



==> acknowledge.tex <==
\newpage
\section*{Acknowledgements}
Parasara Sridhar Duggirala and Edward Kim acknowledge the support of the Air Force Office of Scientific Research under award number FA9550-19-1-0288 and FA9550-21-1-0121 and National Science Foundation (NSF) under grant numbers CNS 1935724 and CNS 2038960. Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the United States Air Force or National Science Foundation. Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the United States Air Force.


==> figures.tex <==


